Transkimmer: Transformer Learns to Layer-wise Skim

Transformer architecture has become the de-facto model for many machine learning tasks from natural language processing and computer vision. As such, improving its computational efficiency becomes paramount. One of the major computational inefficiency of Transformer-based models is that they spend the identical amount of computation throughout all layers. Prior works have proposed to augment the Transformer model with the capability of skimming tokens to improve its computational efficiency. However, they suffer from not having effectual and end-to-end optimization of the discrete skimming predictor. To address the above limitations, we propose the Transkimmer architecture, which learns to identify hidden state tokens that are not required by each layer. The skimmed tokens are then forwarded directly to the final output, thus reducing the computation of the successive layers. The key idea in Transkimmer is to add a parameterized predictor before each layer that learns to make the skimming decision. We also propose to adopt reparameterization trick and add skim loss for the end-to-end training of Transkimmer. Transkimmer achieves 10.97x average speedup on GLUE benchmark compared with vanilla BERT-base baseline with less than 1% accuracy degradation.

==> sec/background.tex <==
\section{Background} \label{sec:background}
\fixme{We won't need the background sec since the ICLR community is already famililar with it. We can frame it as "Problem formulation" or sth like that.}
% \fixme{Transformer}\\
% \fixme{QA task}\\



\textbf{Transformer.} 
The Transformer model adopts the multi-head self-attention mechanism and calculates hidden states for each position as an attention-based weighted sum of input hidden states.
The weight vector is calculated by parameterized linear projection query Q and key K as Equation~\ref{equ:attention}.
Given a sequence of input embeddings, the output contextual embedding is composed by the input sequence with different attention at each position.
\begin{equation} \label{equ:attention}
    \small
    Attn{(Q,K)} = Softmax(\frac{QK^T}{\sqrt{d_k}})
\end{equation}
where $Q, K$ are query and key matrix of input embeddings, $d_k$ is the length of a query or key vector.
The model exploits multiple parallel groups of such attention weights, also referred as attention heads, for attending to information at different positions.
% And BERT further developed the transformer encoder architecture with well-designed pre-training objective and processing encoding for downstream tasks.
% It is pre-trained as a language model by predicting randomly masked tokens and classifying whether the sentences come from the same corpus.
% The Transformer layers are used to generate contextual embeddings and is fine-tuned on downstream tasks with a supervised dataset.
% BERT uses special tokens to encode the different input and output formats uniformly for downstream tasks, such as \benchmark{\small [CLS]} and \benchmark{\small [SEP]}.


% \textbf{Extractive Question Answering.}
% Question answering is one of the ultimate downstream tasks in the NLP.
% It requires the knowledge of word and sentence levels to answer a question according to a text paragraph.
% For given a text document and a question about the context, the answer is a contiguous span of the text.
% BERT uses special tokens to encode the different input and output formats uniformly for downstream tasks. 
% \benchmark{[CLS]} token is appended at the first token as a classification token, which is pooled out for classification downstream tasks.
% \benchmark{[SEP]} token is inserted between sentences or paragraphs to separate different parts of input, e.g. text and question.

